Expressibility in the Lambda Calculus with Letrec

We investigate the relationship between finite terms in lambda-letrec, the lambda calculus with letrec, and the infinite lambda terms they express. As there are easy examples of lambda-terms that, intuitively, are not unfoldings of terms in lambda-letrec, we consider the question: How can those infinite lambda terms be characterised that are lamda-letrec-expressible in the sense that they can be obtained as infinite unfoldings of terms in lambda-letrec? For 'observing' infinite lambda-terms through repeated 'experiments' carried out at the head of the term we introduce two rewrite systems (with rewrite relations) -reg-> and -reg+-> that decompose the term, and produce 'generated subterms' in two notions. Thereby the sort of the step can be observed as well as its target, a generated subterm. In both systems there are four sorts of decomposition steps: -lambda-> steps (decomposing a lambda-abstraction), -@0> and -@1> steps (decomposing an application into its function and argument), and respectively, -del-> steps (delimiting the scope of an abstraction, for -reg->), and -S-> (delimiting of scopes, for -reg+->). These steps take place on infinite lambda-terms furnished with a leading prefix of abstractions for gathering previously encountered lambda-abstractions and keeping the generated subterms closed. We call an infinite lambda-term 'regular'/'strongly regular' if its set of -reg-> -reachable / -reg-> -reachable generated subterms is finite. Furthermore, we analyse the binding structure of lambda-terms with the concept of 'binding-capturing chain'. Using these concepts, we answer the question above by providing two characterisations of lambda-letrec-expressibility. For all infinite lambda-terms M, the following statements are equivalent: (i) M is lambda-letrec-expressible; (ii) M is strongly regular; (iii) M is regular, and it only has finite binding-capturing chains.

==> figs/pstricks/Makefile <==
# create a picture for each file containing a Lagtx fragment in the directory

# disable implicit rules
.SUFFIXES:

TEXFILES=$(wildcard *.tex)

#noflags:
#	make -r default

default: pdfs

pdfs: $(TEXFILES:.tex=.lgr.pdf) $(TEXFILES:.tex=.sgr.pdf) $(TEXFILES:.tex=.ltg-u.pdf) $(TEXFILES:.tex=.ltg-l.pdf) $(TEXFILES:.tex=.ltg-u-bl.pdf) $(TEXFILES:.tex=.ltg-l-bl.pdf)

%.lgr.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/lambdagraph}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%.sgr.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/scopedgraph}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%.ltg-u-bl.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/ltg-bl}' >> $@
	echo '\\newcommand\\nlabel[1]{}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%.ltg-l-bl.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/ltg-bl}' >> $@
	echo '\\newcommand\\nlabel[1]{#1}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%.ltg-u.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/ltg}' >> $@
	echo '\\newcommand\\nlabel[1]{}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%.ltg-l.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/ltg}' >> $@
	echo '\\newcommand\\nlabel[1]{#1}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

include mk/figure.mk


==> figs/pstricks/admissible_abs.tex <==
\lambdaterm{\abs{L}{\abs{x}\nil}}


==> figs/pstricks/admissible_adb.tex <==
\lambdaterm{\abs{Lx}{\s\nil}}


==> figs/pstricks/admissible_app.tex <==
\lambdaterm{\abs{L}{\app{\nil}{\nil}}}


==> figs/pstricks/admissible_var.tex <==
\lambdaterm{\abs{L}{\abs{x}{\nil}}}
\lambdaterm{\abs{Lx}{\var x}}


==> figs/pstricks/cons.tex <==
\lambdaterm{\abs{x}{\letbind{f}{\app
	{\app
		{\s{\op{:}}}
		{\var x}
	}
	{\letvar f}
}}}


==> figs/pstricks/conscons.tex <==
\lambdaterm{\abs{x}{\letbind{f}{\app
	{\app
		{\s{\op{:}}}
		{\vara{x}{0}{180}}
	}
	{\app
		{\app
			{\s{\op{:}}}
			{\var x}
		}
		{\letvar f}
	}
}}}


==> figs/pstricks/consinf.tex <==
\lambdaterm{\abs{x}{\app
	{\app
		{\s{\op{:}}}
		{\var x}
	}
	{\app
	{\app
		{\s{\op{:}}}
		{\var x}
	}
	{\app
	{\app
		{\s{\op{:}}}
		{\var x}
	}
	\etc
	}
	}
}}


==> figs/pstricks/entangled-cpr.tex <==
\lambdaterm{\abs{a}{\abs{b}{\app
		{\abs{c}{\app
			{\abs{d}{\app
				{\etc}
				{\cpr{d}{\cpR{a}{\var c}}}
			}}
			{\cpr{a}{\cpR{c}{\var b}}}
		}}
		{\cpr{b}{\var a}}
}}}


==> figs/pstricks/entangled-cpreager.tex <==
\lambdaterm{\abs{a}{\abs{b}{\app
		{\cpr{a}\nil}
		{\cpr{b}{\var a}}
}}}


==> figs/pstricks/entangled.tex <==
\lambdaterm{\abs{a}{\abs{b}{\app
		{\abs{c}{\app
			{\abs{d}{\app
				{\etc}
				{\s{\var c}}
			}}
			{\s{\var b}}
		}}
		{\s{\var a}}
}}}


==> figs/pstricks/lx_xx.tex <==
\lambdaterm{\abs{x}{\app{\vara{x}{180}{180}}{\var x}}}


==> figs/pstricks/lx_xx_shared.tex <==
\lambdaterm{\abs{x}{\app{\letbind{f}{\vara{x}{180}{180}}}{\letvara{f}{180}{0}}}}


==> figs/pstricks/lxy_xxy-cpreager.tex <==
\lambdaterm{\abs{x}{\abs{y}{\app{\cpr{y}{\app{\var x}{\var x}}}{\cpR{x}{\var y}}}}}


==> figs/pstricks/lxy_xxy-cprgraph.tex <==
\lambdaterm{\abs{x}{\abs{y}{\app{\cprapp{y}{\app{\var x}{\var x}}{\cpr{y}{\var x}}{\cpr{y}{\var x}}}{\cpr{x}{\var y}}}}}


==> figs/pstricks/lxy_xxy-cprlazy.tex <==
\lambdaterm{\abs{x}{\abs{y}{\app{\app{\cpr{y}{\var x}}{\cpR{y}{\var x}}}{\cpr{x}{\var y}}}}}


==> figs/pstricks/lxy_xxy-eager.tex <==
\lambdaterm{\abs{x}{\abs{y}{\app{\s{\app{\var x}{\var x}}}{\var y}}}}


==> figs/pstricks/lxy_xxy-lazy.tex <==
\lambdaterm{\abs{x}{\abs{y}{\app{\app{\s{\var x}}{\s{\var x}}}{\var y}}}}


==> figs/pstricks/lxy_xxy-redgraph.tex <==
\lambdaterm{\abs{x}{\abs{y}{\app{\sapp{\app{\var x}{\var x}}{\s{\var x}}{\s{\var x}}}{\var y}}}}


==> figs/pstricks/lxy_xxy-regmin.tex <==
\lambdaterm{\abs{x}{\abs{y}{\app{\app{\var x}{\var x}}{\var y}}}}


==> figs/pstricks/macros/lambdagraph.tex <==
% Named Lambda Graph with Invisible Scopes

\newcommand\tree[2]{\pstree[linewidth=0.5pt,nodesep=0.4mm,levelsep=0.8cm]{#1}{#2}}
\newcommand\node[1]{\TR{#1}}

% The Language

\newcommand\lambdaterm[1]{\ensuremath{\tree{\nil}{#1}}}

\newcommand\letbind[2]{\rnode[t]{#1}{#2}}
% with explicit sharing node
%\newcommand\letbind[2]{\tree{\node{\rnode[t]{#1}{\vphantom{i}\pstriangle(0mm,3.28mm)(6mm,-3.9mm)}}}{#2}}
\newcommand\letvar[1]{{\psset{nodesepB=0pt}\Tp*[name=here]}\ncangles[nodesepA=0pt,angleB=70]{-}{here}{#1}}
\newcommand\letvara[3]{{\psset{nodesepB=0pt}\Tp*[name=here]}\ncangles[nodesepA=0pt,angleA=#2,angleB=#3]{-}{here}{#1}}
\newcommand\abs[2]{\tree{\node{\lambda #1}}{#2}}
\newcommand\s[1]{#1}
\newcommand\sA[1]{#1}
\newcommand\cpr[2]{#2}
\newcommand\cpR[2]{#2}
\newcommand\app[2]{\tree{\node{@}}{#1 #2}}
\newcommand\var[1]{\node{#1}}
\newcommand\vara[3]{\node{#1}}

\newcommand\sapp[3]{\app{#2}{#3}}
\newcommand\cprapp[4]{\app{#3}{#4}}

\newcommand\etc[0]{\node{\vdots}}
\newcommand\op[1]{\Tcircle{#1}}
\newcommand\nil{\node{}}


==> figs/pstricks/macros/ltg-bl.tex <==
% Lambda Transition Graph with Back-Links

% CAUTION: The lambda-letrec constructors are supposed to be used as unsaturated functions.
%          The last two parameters are all supplied here.
%          First paramater: labelling of the incoming edge
%          Second paramater: labelling of this node

\newcommand\mkNode\Toval
\newcommand\putEdge{\mput*}
\newcommand\tree[2]{\pstree[arrows=->,treesep=1cm,levelsep=1.5cm]{#1}{#2}}
\newcommand\node[1]{\mkNode{\nlabel{#1}}}


% The Language

%\newcommand\lambdaterm[1]{\ensuremath{\tree{\TR{}}{#1{}{}}}}
\newcommand\lambdaterm[1]{\ensuremath{#1{}{}}}

\newcommand\app[4]{\tree{\node{#4}#3}{#1{\putEdge{@_0}}{#4} #2{\putEdge{@_1}}{#4}}}

\newcommand\abs[4]{\tree{\rnode{#1}{\node{#4}}#3}{#2{\putEdge\lambda}{#4#1}}}

\newcommand\s[3]{
	\StrGobbleRight{#3}1[\NewStr]
	\tree{\node{#3}#2}{#1{\putEdge S}\NewStr}
}

\newcommand\sA[3]{
	\StrGobbleRight{#3}1[\NewStri]
	\tree{\node{#3}#2}{#1{\putEdge S}\NewStri}
}

\newcommand\sapp[5]{
	\StrGobbleRight{#5}1[\NewStri]
	\tree{\node{#5}#4}{#1{\putEdge S}\NewStri #2{\putEdge{@_0}}{#5} #3{\putEdge{@_1}}{#5}}
}

\newcommand\cprapp[6]{
	\StrDel[1]{#6}{#1}[\ANewStrin]
	\tree{\node{#6}#5}{#2{\putEdge{del}}\ANewStrin #3{\putEdge{@_0}}{#6} #4{\putEdge{@_1}}{#6}}
}

\newcommand\cpr[4]{
	\StrDel[1]{#4}{#1}[\NewStrin]
	\tree{\node{#4}#3}{#2{\putEdge{del}}\NewStrin}
}

\newcommand\cpR[4]{
	\StrDel[1]{#4}{#1}[\NewString]
	\tree{\node{#4}#3}{#2{\putEdge{del}}\NewString}
}

\newcommand\var[3]{{\psset{nodesepB=0pt}\mkNode[name=here]{\nlabel{#3}}#2}\ncangles[nodesepA=0pt]{->}{here}{#1}\ncput*{0}}
\newcommand\vara[5]{{\psset{nodesepB=0pt}\mkNode[name=here]{\nlabel{#5}}#4}\ncangles[nodesepA=0pt,angleA=#2,angleB=#3]{->}{here}{#1}\ncput*{0}}

\newcommand\etc[2]{\TR{\vdots}#1}

\newcommand\letbind[4]{#2{\rnode{#1}{}#3}{#4}}

\newcommand\letvar[3]{{\psset{arrows=-,nodesepB=0pt}\Tp*[name=here]}\ncangles[angleB=70,nodesepA=0pt]{->}{here}{#1}#2}
\newcommand\letvara[5]{{\psset{arrows=-,nodesepB=0pt}\Tp*[name=here]}\ncangles[angleA=#2,angleB=#3,nodesepA=0pt]{->}{here}{#1}#4}

%\newcommand\op[3]{\tree{\node{#3}#2}{\mkNode{#1}}}
%\newcommand\op[3]{\var{#1}{#2}{#3}}
%\newcommand\op[3]{\etc{#2}{#3}}
\newcommand\op[3]{\TR{\dots}#2}

\newcommand\nil[2]{\node{#2}#1}


==> figs/pstricks/macros/ltg.tex <==
% The Lambda Transition Graph without Back-Links

\input{macros/ltg-bl}

\renewcommand\var[3]{\tree{\node{#3}#2}{}}
\renewcommand\vara[5]{\tree{\node{#5}#4}{}}


==> figs/pstricks/macros/scopedgraph.tex <==
% Nameless Lambda Graph with Visible Scopes

\input{macros/lambdagraph}

\renewcommand\abs[2]{\tree{\node{\lambda}}{#2}}
\renewcommand\s[1]{\tree{\node S}{#1}}
\renewcommand\var[1]{\node{0}}
\renewcommand\vara[3]{\node{0}}


==> figs/pstricks/mk/postlude.tex <==
\end{document}


==> figs/pstricks/simpleletrec-eager.tex <==
% λx.letrec f = λy.f yx in f ]

\lambdaterm{\letbind{f}{\abs{x}{\abs{y}{\app{\app{\s{\sA{\letvara{f}{180}{100}}}}{\var y}}{\s{\var x}}}}}}


==> figs/pstricks/simpleletrec-lazy.tex <==
% λx.letrec f = λy.f y x in f ]

\lambdaterm{\abs{a}{\abs{b}{\app{\app{
	\abs{c}{\abs{d}{\app{\app{
		\etc
	}{\var d}}{\s{\var c}}}}
}{\var b}}{\s{\var a}}}}}


==> figs/pstricks/var.tex <==
\lambdaterm{\app{\abs{x}{\abs{z}{\app{\s{\vara{x}{180}{180}}}{\var z}}}}{\abs{y}{\abs{w}{\app{\app{\s{\vara{y}{180}{180}}}{\var w}}{\s{\var y}}}}}}
%\lambdaterm{\app{\abs{x}{\abs{z}{\app{\s{\zero}}{\zero}}}}{\abs{y}{\abs{w}{\app{\app{\s{\zero}}{\zero}}{\s{\zero}}}}}}


==> lDFAs.tex <==
Things to develop here:
\begin{itemize}
  \item Explain that the notion of \lTG\ from Section~\ref{sec:letrec2} 
    has a drawback: on bisimulation collapses of such \lTG{s}, extended scopes are not
    nested nicely any more. Give example.
  \item Remedy: define variant \lTG{s} with $\nlvar$\nb-backlinks to `abstraction nodes'.
  \item Introduce these, in the finite case, as \lDFA{s}.  
  \item Show that nesting of extended scopes is preserved under bisimulation collapse for the new version.
  \item `admissible' \lTG: an \lTG\ that is bisimilar to the \lTG\ of a term in $\lambdaletreccal$.
  \item recognition of admissibility for \lTG{s}/\lDFA{s} is decidable in linear time.
  \item `tight-(extended-)scope admissible' \lTG: an an \lTG\ that is bisimilar 
    to the `tight-(extended-)scope-\lTG\ of a term in $\lambdaletreccal$.  
  \item \todo{Conjecture:} recognition of tight-scope admissibility of an \lDFA\ is decidable in quadratic time.   
\end{itemize}


In this section we develop an efficient method to increase sharing in a
\lambdaletrec{}-term. It relies on a a variant of $\lambda$-transition graphs,
called \emph{\lDFA}s. Like a $\lambda$-transition graph a \lDFA is a graphical
representation of a term, but only for the latter can the bisimulation collapse
directly interpreted as a \lambdaletrec{}-term.

%The following example demonstrates that for \lTG{s} as defined in Section~\ref{sec:letrec2}
%scopes of abstractions are not preserved under bisimulation.

\todo{Voorbeeld gaat verhuizen (op kamers) naar sectie maximal sharing.}

\begin{example}\protect\label{ex:scopes:not:nested}
  Consider the $\lambda$-term
  $\ater=\lapp{(\labs{\avar}{\labs{\cvar}{\lapp{\avar}{\cvar}}})}{\labs{\bvar}{\lapp{\labs{w}{\lapp{\bvar}{w}}}{\bvar}}}$
  and its tight-scope \lTG. Next to it is its bisimulation collapse, but with
  the node labels removed beforehand, since we need to capture
  \emph{structural} repetition which should not be disturbed by the choice of
  names for the variables: \todo{See Figure~\ref{fig:labels}.}
  \begin{figure}[t]
    \fig{pstricks/var.ltg-l} \hspace{1cm} \fig{pstricks/var.ltg-u}
    \caption{\label{fig:labels}\todo{Den Kollaps werde ich später noch von Hand durchführen}}
  \end{figure}
  Let us try to interpret the collapsed graph as a $\lambdaletrec$-term.
  That means, we have to express the sharing that occurs in the graph via a
  $\sletrec$, which cannot be done since the scopes of the binders
  $\labsbind\avar$ and $\labsbind\bvar$ from outside of the shared expression
  would come to overlap, which is not supported by $\lambdaletreccal$.
\end{example}

The example illustrates that this straightforward approach induces a notion of
sharing that is too strong for the $\lambdaletrec$-calculus. In order to
weaken the sharing introduced by the collapse we impose additional structure to
the \lTG: $\snlvar$-edges do no longer point to a leaf node but point
back to the node whose $\slabsdecomp$-successor's label has the variable in
question as its rightmost component. 
\todo{Zeigen, dass diese eindeutig definiert sind.}

\begin{example}
  The unlabelled \lTG~of Example \ref{ex:scopes:not:nested} equipped with
  \emph{$\snlvar$-backlinks} cannot be collapsed and therefore does not
  introduce to sharing which is expressible in $\lambdaletreccal$:
  See Figure~\ref{fig:backlinks}:
  \begin{figure}[t]
    \fig{pstricks/var.ltg-l-bl} \hspace{1cm} \fig{pstricks/var.ltg-u-bl}
    \caption{\label{fig:backlinks}\ldots.}
  \end{figure}  
\end{example}

We call such an unlabelled \lTG with $\snlvar$-backlinks a \lDFA. \lDFA{s}
are finite state automata with labels of transitions in \lTG{s} as input
symbols.

\begin{definition}[\lDFA{s}]
  A \emph{\lDFA} is a DFA~$\aDFA =
  \tuple{\DFAstates,\inputalph,\transfunc,\startstate,\finalstates}$ with input
  alphabet $ \setexp{\slabstrans, \slappitrans{0}, \slappitrans{1}, \ssucctrans, \szerotrans} \subseteq \inputalph $
  and $\finalstates = \emptyset$, an empty set of final states.  
\end{definition}

%It is straightforward to interpret a $\lambda$-transition graph of a term ($\in
%\iTer\lambdacal \cup \Ter\lambdaletreccal)$ as a \lDFA by omitting all node
%labels.

Now we're gonna define a readback function \srb. But first we need to define
the domain of that function.

\begin{definition}[Admissible {\lDFA}s]
We call a \lDFA{} \emph{admissible} if there is a labelling of its nodes such
that the label of the start node is empty and every node $n$ falls in one of
the following categories:

\begin{tabular}{ccccccc}
\fig{pstricks/admissible_app.ltg-l}
&
\fig{pstricks/admissible_abs.ltg-l}
&
\fig{pstricks/admissible_adb.ltg-l}
&
\fig{pstricks/admissible_var.ltg-l-bl}
\\
(1)&(2)&(3)&(4)
\todo{Muss noch von Hand richtig zusammengesetzt werden}
\end{tabular}

\begin{enumerate}
\item Application: Precisely two outgoing edges labelled $\slappitrans0$ and $\slappitrans1$.
The node labels of $n$'s successors' are identical to $n$'s label.
\item Abstraction: A single outgoing edge labelled $\slabstrans$ connecting $n$ to a node whose label
extends $n$'s label by an additional variable.
\item Adbmal: $n$ has at least one variable in its label and a single outgoing
$\ssucctrans$-edge pointing to a node with the same label, except for rightmost
variable which is missing.
\item Variable: $n$ has at least one variable in its label and a single
outgoing $\snlvar$-edge pointing to a node $m$ with the same label except
for the rightmost variable $x$ which is missing. $m$ in turn is an abstraction node that
introduces $x$.
\end{enumerate}
\end{definition}

The following system is a modification of the rules from
Definition~\ref{def:decompreds} such that $\snlvar$-transitions point back
to their respective $\lambda$\nb-abstraction.

\begin{definition}

  \begin{align*}
    (\srulep{\slappdecompi{i}}): 
      & &
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n}^{\biteri{n}}}{\lapp{\ateri{0}}{\ateri{1}}}
      & {} \red %\lappdecompi{i}
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n}^{\biteri{n}}}{\ateri{i}}  
      & & \hspace*{-0.5ex} (i\in\{0,1\})
    \\
    (\srulep{\slabsdecomp}):
      & &
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n}^{\biteri{n}}}{\labs{\avari{n+1}}{\aiteri{0}}}
      & {} \red %\labsdecomp
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n}^{\biteri{n}}\avari{n+1}^{\aiteri{0}}}{\aiteri{0}} 
    \displaybreak[0]\\
    (\srulep{\snlvarsucc}):
      & &
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n}^{\biteri{n}}}{\aiteri{0}}
      & {} \red %\compressstreg
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n-1}^{\biteri{n-1}}}{\aiteri{0}}  
      %& & \hspace*{-0.5ex} %(\text{if }\avari{n}\notin\freevars{\ater})
    %\\  
      & & 
      \hspace*{-9ex}
                           (\text{if binding }\flbind{\avari{n}}\text{ is vacuous})
    \displaybreak[0]\\  
    (\srulep{\scompress}):
      & &
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n}^{\biteri{n}}}{\aiteri{0}}
      & {} \red %\compresstreg
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{i-1}^{\biteri{i-1}}\avari{i+1}^{\biteri{i+1}}\ldots\avari{n}^{\biteri{n}}}{\aiteri{0}}   
      & & 
    \\   
      & & & & &
      \hspace*{-9ex} %(\text{if }\avari{i}\notin\freevars{\labs{\avari{i+1}\ldots\avari{n}}{\ater}})
                        (\text{if binding }\flbind{\avari{i}}\text{ is vacuous})
    \displaybreak[0]\\
    (\srulep{\snlvar}):
      & &
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n+1}^{\biteri{n+1}}}{\avari{n+1}}
      & {} \red
    \flabs{\avari{1}^{\biteri{1}}\ldots\avari{n}^{\biteri{n}}}{\labs{\avari{n+1}}{\biteri{n+1}}}   
%     \\
%     (\srulep{i}):
%       & &
%     \femptylabs{\avarnamei{i}}
%       & {} \red
%     \femptylabs{\stopsymb{\avarnamei{i}}}   
%       & & \hspace*{-0.5ex} (i\in\nats)      
    %
  \end{align*}
  
  \todo{Ask Vincent on how to best represent this system as a HRS:
        I would tend to use product ($\times$) types (possible in HRSs (via coding)?).}
\end{definition}  
% 
%   \begin{align*}
%     (\srulep{\slappdecompi{i}}): 
%       & & \hspace*{-25ex}
%     \flabsHRS{n}{\avari{1}\ldots\avari{n}}{\lapp{\cmetavari{0}{\vec{\avar}}}{\cmetavari{1}{\vec{\avar}}}}
%       & {} \red 
%     \flabsHRS{n}{\avari{1}\ldots\avari{n}}{\cmetavari{i}{\vec{\avar}}}  
%       \hspace*{4ex} (i\in\{0,1\})
%     \\
%     (\srulep{\slabsdecomp}):
%       & & 
%     \flabsHRS{n}{\avari{1}\ldots\avari{n}}{\labs{\avari{n+1}}{\cmetavar{\vec{\avar}}}}
%       & {} \red 
%     \flabsHRS{n}{\avari{1}\ldots\avari{n+1}}{\cmetavar{\vec{\avar}}} 
%     \displaybreak[0]\\
%     (\srulep{\snlvarsucc}):
%       & & 
%     \flabsHRS{n}{\avari{1}\ldots\avari{n}}{\cmetavar{\avari{1},\ldots,\avari{n-1}}}
%       & {} \red 
%     \flabsHRS{n-1}{\avari{1}\ldots\avari{n-1}}{\cmetavar{\avari{1},\ldots,\avari{n-1}}}
%     \displaybreak[0]\\  
%     (\srulep{\scompress}):
%       & & & \hspace*{-35ex}
%       \begin{aligned}
%         & 
%         \flabsHRS{n}{\avari{1}\ldots\avari{n}}{\cmetavar{\avari{1},\ldots,\avari{i-1},\avari{i+1},\ldots,\avari{n-1}}}
%         \red
%         \\
%         & \hspace*{16ex} 
%         \flabsHRS{n-1}{\avari{1}\ldots\avari{i-1}\avari{i+1}\ldots\avari{n}}{\cmetavar{\avari{1},\ldots,\avari{i-1},\avari{i+1},\ldots,\avari{n-1}}}
%       \end{aligned}
%     \displaybreak[0]\\  
%     (\srulep{\snlvar}):
%       & &
%     \flabsHRS{n}{\vec{\avar}\bvar}{\bvar}
%       & {} \red
%     \flabsHRS{n}{\vec{\avar}\bvar}{\stopsymb{\bvar}}   
%     \\
%     (\srulep{i}):
%       & &
%     \femptylabsHRS{\avarnamei{i}}
%       & {} \red
%     \femptylabsHRS{\stopsymb{\avarnamei{i}}}   
%       \hspace*{8ex} (i\in\nats)            
%     %
%   \end{align*}
  
\begin{proposition}
\todo{There is a bisimulation between the original derivations and derivations using the backlinks.}
\end{proposition}

\begin{proposition}
The unlabelled transition graph of this system is an admissible \lDFA{}.
\end{proposition}



==> maximal.tex <==
Motivation:
When used to express computations, the \sletrec{} structure of a
\lambdaletrec-term is still of interest for two reasons. Firstly, in a
\lambdaletrec-based programming language (most functional programming
languages) one representation may be considered better programming style than
another. Secondly, the \sletrec{} structure often directly influences the
representation of the term in the memory of the executing machine, and the
sharing structure specifically which affects execution efficiency.

Things to put here:
\begin{itemize}
  \item define `maximal sharing' for $\lambda$- and $\lambdaletrec$\nb-terms 
     \todo{read in Hasegawa's thesis \cite{hase:1997}}
     \begin{itemize}
       \item \todo{Abbildungen zu Graphen hin.} 
     \end{itemize}   
     
     
  \item reading back $\lambdaletrec$\nb-terms from tight-scope admissible \lDFA{s} \todo{in linear time?}
  \item reading back $\lambdaletrec$\nb-terms admissible \lDFA{s} \todo{in quadratic time?} 
  \item Main Theorem: Maximal Sharing in a $\lambdaletrec$\nb-term can be obtained \todo{in quadratic time?}:
    \begin{itemize}
      \item translation into a tight-scope \lDFA\ (quadratic time?)
      \item minimisation of the tight-scope \lDFA\ (in $\bigO{n\log n}$ time)
      \item readback of maximally shared $\lambdaletrec$\nb-term (in $\bigO{n}$ time)
    \end{itemize}   
   
    
\end{itemize}

Here we develop the means to compare the \emph{degree of sharing} of two terms
leading to a proper definition of \emph{maximal sharing}. Problem: e.g.~for
\lambdaletreccal{} we want to ignore the freedom of placing binding at different positions.
Therefore we express sharing by means of a mapping from terms to an LTS. The
mapping is an interpretation function which interprets the sharing in the term.

\begin{example}Four possible interpretations of $\labs{x}{\lapp xx}$:\\
%\fig{pstricks/lx_xx.ltg-l} \fig{pstricks/lx_xx_shared.ltg-l}
%\fig{pstricks/lx_xx.ltg-l-bl} \fig{pstricks/lx_xx_shared.ltg-l-bl}
\end{example}

It is natural (yet not essential) to require of such an interpretation function $I$:
  $I(\ateri1) \bisim I(\ateri2) \Longrightarrow \ateri1 = \ateri2$.

\begin{definition}[bisimulation step]
We write $A \bisimstep B$ when $A \bisim B$ and $B$ can be obtained from $A$ by
contrating two of its nodes.
\end{definition}

\begin{remark}
$\sbisim = (\leftrightsquigarrow)^*$
\end{remark}

\begin{definition}[sharing degree for LTSs]
Let us define a partial order on LTSs for comparing their degree of sharing. We
write $\aLTS \leq \bLTS$ iff $\bLTS \bisimstep^* \aLTS$ and we say that $\aLTS$ has a higher degree of sharing than $\bLTS$.
\end{definition}

\begin{definition}[sharing degree for terms]
We can propagate the degree of sharing to terms. For some interpretation
function $I$ we write $\ater \leq_I \bter$ iff $I(\ater) \leq I(\bter)$ and say
$\ater$ has a higher degree of sharing (w.r.t.~$I$) than $\bter$.
\end{definition}

\begin{proposition}[Readback correctness]
  Let $d$ be a \lDFA. If $d$ is admissible and its readback is $rb{d}\in\iTer\lambdaletreccal$ then
  $\exists \ateri1\in\iTer\lambdacal : rb(d) \infred_{\unfold\alpha} \ateri{1} \land \ltg\sastratred{\ateri1} \bisim d$.
\end{proposition}

\begin{example}
  \todo{This example is intended to indicate that bisimulation collapse is most effective for tight-scope versions of \lTG{s} of terms in $\lambdaletreccal$}
  \begin{itemize}
    \item 
      $\labs{\cvar}{\lapp{(\labs{\avar}{\lapp{(\labs{\bvar}{\lapp{\cvar}{\bvar}})}{\avar}})}{\labs{\fvar}{\lapp{\cvar}{\fvar}}}}$
    \item 
      $\nllabs{\nllapp{(\nllabs{\nllapp{(\nllabs{\nllapp{(\nlvarsucc{\nlvarsucc{\nlvar}})}{\nlvar}})}{\nlvar}})}
                      {\nllabs{(\nllapp{\nlvarsucc{\nlvar})}{\nlvar}}}}$ 
      de~Bruijn index translation,
      does not allow to increase sharing under bisimulation collapse
    \item 
      $\nllabs{\nllapp{(\nllabs{\nllapp{(\nlvarsucc{\nllabs{\nllapp{(\nlvarsucc{\nlvar})}{\nlvar}}})}{\nlvar}})}
                      {\nllabs{(\nllapp{\nlvarsucc{\nlvar})}{\nlvar}}}}$,
      `lazy' nameless version, does allow to increase sharing under bisimulation collapse, namely: 
    \item 
      $\nllabs{(\letrec{\arecvar = \nllabs{\nllapp{(\nlvarsucc{\nlvar})}{\nlvar}}}
                       {\nllapp{(\nllabs{\nllapp{(\nlvarsucc{\arecvar})}{\nlvar}})}{\arecvar}}
                )}$,
      or:
    \item 
      $\labs{\cvar}{\letrec{\arecvar = \labs{\bvar}{(\lapp{(\nlvarsucc{\cvar})}{\bvar}}}
                           {\nllapp{(\labs{\avar}{\nllapp{(\nlvarsucc{\arecvar})}{\avar}})}{\arecvar}}}$,
        the named version. 
  \end{itemize}
  
  
  
  
\end{example}


==> readback.tex <==

% Rough, but impressive tunes by the MC G Family, T,D,G Producoes: http://youtu.be/pLGq1W2mBpQ http://youtu.be/7t_3pmII2kY http://youtu.be/pgpE1gpYcmc 
% Elizio Feat Mika Mendes - Put It Down http://youtu.be/3uaf1NR3Gjg




%  
% \newcommand{\sreadback}{\textsf{readback}}
% \newcommand{\readback}{\funap{\sreadback}}
% \newcommand{\sreadwriten}{\indap{\textsf{rw}}}
% \newcommand{\readwriten}[1]{\bfunap{\sreadwriten{#1}}}
% \newcommand{\sreadwritezero}{\indap{\textsf{rw}}{0}}
% \newcommand{\readwritezero}{\funap{\sreadwritezero}}

% Readback function $\sreadback \funin \iTer{\setexp{\nlvarfo, \snllabsfo, \snllappfo, \snlvarsuccfo }} \to \Ter{\inflambdacal}$
% defined by: $\bnllter \mapsto \readback{\bnllter} \defdby $ infinite normal form of $\readwritezero{\bnllter}$ w.r.t.\ the following CRS:
% \todo{Unendliche S-Ketten ausschließen? Zusammenhang zu \lambda-Transitionsgraphen herstellen}
% %
% \begin{align*}
%   \readwriten{n}{\sametavari{1},\ldots,\sametavari{n}}{\nllabsfo{\bnllteri{0}}}
%     & {} \;\red\;
%   \labsCRS{\avar}{\readwriten{n+1}{\sametavari{1},\ldots,\sametavari{n},\avar}{\bnllteri{0}}}  
%   \\
%   \readwriten{n}{\vec{\sametavar}}{\nllappfo{\bnllteri{0}}{\bnllteri{1}}}
%     & {} \;\red\;
%   \lappCRS{\labsCRS{\avar}{\readwriten{n}{\vec{\sametavar}}{\bnllteri{0}}}}
%           {\labsCRS{\avar}{\readwriten{n}{\vec{\sametavar}}{\bnllteri{1}}}}
%   \\
%   \readwriten{n+1}{\vec{\sametavar},\avar}{\nlvarsuccfo{\bnllteri{0}}}
%     & {} \;\red\;
%   \readwriten{n}{\vec{\sametavar}}{\bnllteri{0}}
%   \\
%   \readwriten{n}{\sametavari{1},\ldots,\sametavari{n}}{\nlvarfo}
%     & {} \;\red\;
%   \sametavari{n}
% \end{align*}


Motivation for the decomposition functions on abstraction prefix terms: 
%
\begin{align*}
  \parsen{n}{\vecsub{\sametavar}{n}}{\flabsCRS{n}{\vecsub{\avar}{n}}{\labsCRS{\bvar}{\cmetavar{\vecsub{\avar}{n},\bvar}}}}
    & {} \;\red\;
  \labsCRS{\bvar}{\parsen{n+1}{\vecsub{\sametavar}{n},\bvar}{\flabsCRS{n+1}{\vecsub{\avar}{n}}{\absCRS{\bvar}{\cmetavar{\vecsub{\avar}{n},\bvar}}}}}
  \\
  \parsen{n}{\vecsub{\sametavar}{n}}{\flabsCRS{n}{\vecsub{\avar}{n}}{\lappCRS{\cmetavari{0}{\vecsub{\avar}{n}}}{\cmetavari{1}{\vecsub{\avar}{n}}}}}  
    & {} \;\red\;
  \lappCRS{\parsen{n}{\vecsub{\sametavar}{n}}{\flabsCRS{n}{\vecsub{\avar}{n}}{\cmetavari{0}{\vecsub{\avar}{n}}}}}{\parsen{n}{\vecsub{\sametavar}{n}}{\flabsCRS{n}{\vecsub{\avar}{n}}{\cmetavari{1}{\vecsub{\avar}{n}}}}}  
  \\
  \parsen{n+1}{\sametavari{1},\ldots,\sametavari{n+1}}{\funap{\sflabsCRS{n+1}}{\absCRS{\vecsub{\avar}{n+1}}{\cmetavar{\vecsub{\avar}{n}}}}}
    & {} \;\red\;
  \parsen{n}{\sametavari{1},\ldots,\sametavari{n}}{\funap{\sflabsCRS{n}}{\absCRS{\vecsub{\avar}{n}}{\cmetavar{\vecsub{\avar}{n}}}}}
  \\
  \parsen{n}{\sametavari{1},\ldots,\sametavari{n}}{\flabsCRS{n}{\vecsub{\avar}{n}}{\avari{n}}}
    & {} \;\red\;
  \sametavari{n}
\end{align*}

\begin{proposition}
  For every term $\aiter\in\Ter{\lambdacal}$ it holds:
  \begin{equation*}
    \parseempty{\femptylabs{\aiter}} \infred_{parse} \aiter
  \end{equation*}
\end{proposition}


\begin{proposition}
  For every term $\allter\in\Ter{\lambdaletreccal}$ and $\aiter\in\Ter{\inflambdacal}$ it holds:
  \begin{equation*}
    \parseempty{\femptylabs{\allter}} \infred_{\sunf,parse} \aiter
      \;\;\;\;\;\;\Longleftrightarrow\;\;\;\;\;\;
    \allter \unfoldinfred \aiter  
  \end{equation*}
\end{proposition}


A \lambdaletrec\nb-term~$\allter$ is \emph{$\llunfCRS$\nb-productive}
if it expresses an infinite \lambdaterm. 


Let $\astrat$ be a strategy for $\RegletrecARS$.
$\allter$ is called \emph{productive with respect to $\sstratred{\astrat}$}
if in all $\sstratred{\astrat}$\nb-rewrite sequences on $\allter$ \ldots.



\begin{proposition}
%   A \lambdaletrec\nb-term~$\allter$ is $\llunfCRS$\nb-productive
%    if and only if
%   there is a \scopedelimiting\ strategy~$\astrat$ for $\RegletrecARS$ 
%   such that every $\astrat$\nb-normal forms of $\allter$ is also a normal form of $\RegARS$
%   (and hence of the form $\flabs{\avari{1}\ldots\avari{n}}{\avari{n}}$.)  
  For all \lambdaletrec\nb-terms~$\allter$ the following statements are equivalent:
  \begin{enumerate}[(i)]
    \item 
      $\allter$ is $\llunfCRS$\nb-productive.
    \item 
      There is a \scopedelimiting\ strategy~$\astrat$ for $\RegletrecARS$ 
      such that $\allter$ is productive with respect to $\stratred{\astrat}$. 
%       such that every $\astrat$\nb-normal forms of $\allter$ is also a normal form of $\RegARS$
%       (and hence of the form $\flabs{\avar}{\avar}$.) 
%     \item 
%       There is a \extscopedelimiting\ strategy~$\astratplus$ for $\RegletrecARS$ 
%       such that every $\astratplus$\nb-normal forms of $\allter$ is also a normal form of $\RegARS$
%       (and hence of the form $\flabs{\avari{1}\ldots\avari{n}}{\avari{n}}$.) 
  \end{enumerate}
  
  
  
  
\end{proposition}


